CBench: Towards Better Evaluation of Question Answering Over Knowledge Graphs

Recently, there has been an increase in the number of knowledge graphs that can be only queried by experts. However, describing questions using structured queries is not straightforward for non-expert users who need to have sufficient knowledge about both the vocabulary and the structure of the queried knowledge graph, as well as the syntax of the structured query language used to describe the user's information needs. The most popular approach introduced to overcome the aforementioned challenges is to use natural language to query these knowledge graphs. Although several question answering benchmarks can be used to evaluate question-answering systems over a number of popular knowledge graphs, choosing a benchmark to accurately assess the quality of a question answering system is a challenging task. In this paper, we introduce CBench, an extensible, and more informative benchmarking suite for analyzing benchmarks and evaluating question answering systems. CBench can be used to analyze existing benchmarks with respect to several fine-grained linguistic, syntactic, and structural properties of the questions and queries in the benchmark. We show that existing benchmarks vary significantly with respect to these properties deeming choosing a small subset of them unreliable in evaluating QA systems. Until further research improves the quality and comprehensiveness of benchmarks, CBench can be used to facilitate this evaluation using a set of popular benchmarks that can be augmented with other user-provided benchmarks. CBench not only evaluates a question answering system based on popular single-number metrics but also gives a detailed analysis of the linguistic, syntactic, and structural properties of answered and unanswered questions to better help the developers of question answering systems to better understand where their system excels and where it struggles.

==> sections/Old_Evaluation.tex <==
=============End of Section=====================




% In this section, we deeply evaluated different QA systems concerning the questions and their queries properties. For this evaluation, we first categorized the questions based on their queries shapes. After that, we feed the QA system by the questions from a specific benchmark and collect the answers. These answers are compared to the correct ones to compute the \emph{True Positive} (\emph{TP}), \emph{False Positive} (\emph{FP}) and \emph{False Negative} (\emph{FN}). Then, these measures are used to compute the \emph{Recall} and \emph{Precision} as follow
% \[Recall = \frac{TP}{TP + FP}\] and \[Precision = \frac{TP}{TP + FN}\]

% The first system used for this evaluation is \emph{gAnsewr}~\cite{hu2017answering} which fed by questions from \emph{QALD 6}, a one that is used in its original evaluation. Figure  \ref{fig:PR} shows the \emph{Recall} and \emph{Precision} for every set of questions in which their queries are belonging to a specific shape. Excluding the \emph{Cycle} shape because only two questions are belonging to it, \emph{Single-Edge} has the highest \emph{Recall} and \emph{Precision}. It was expected because it is the simplest type of questions. When the shape contains the \emph{Single-Edge} along with other complex questions as in \emph{Chain}, \emph{Chain Set}, \emph{Tree}, \emph{Forest}, \emph{Flower} and \emph{Flower Set}, the percentages of \emph{Precision} and \emph{Recall} decreased. The \emph{Star} shape is a special case of the \emph{Tree} shape and it has the smallest \emph{Precision} and \emph{Recall}.

% \begin{figure}[tbp]
%   \includegraphics[width=0.85\linewidth]{figures/PR.png}
%   \caption{Recall and Precision Analysis for gAnswer and WDAqua-core1 Systems with respect to Queries Shapes.}
%   \label{fig:PR}
% \end{figure}



\begin{figure}[tbp]
  \includegraphics[width=0.9\linewidth]{figures/gAnswerChain.png}
  \caption{Chain Questions Answered by gAnswer for Different Properties.\comment{For this and following figures, consider shortening the text. For example, (CQ, select-distinct, T=1). Also, consider putting all different shapes figures as subfigures in one figure.}}
  \label{fig:gAnswerChain}
\end{figure}

\begin{figure}[tbp]
  \includegraphics[width=0.9\linewidth]{figures/gAnswerStar.png}
  \caption{Star Questions Answered by gAnswer for Different Properties.}
  \label{fig:gAnswerStar}
\end{figure}



To deeply check the questions that the system can answer and those cannot be answered, we made a question by question analysis. For every question, we determined its query properties like triples' category, queries' keywords and the number of triples. This analysis is made separately for every query shape type and we aggregated the questions that have the same properties. As an example here, Figure \ref{fig:gAnswerChain} and \ref{fig:gAnswerStar} show the properties for the questions' queries for \emph{Chain} and \emph{Star} shapes, respectively. The figures also show how many questions of every set of properties answered by \emph{gAnswer} and how many of them cannot be answered.

In Figure \ref{fig:gAnswerChain}, we selected the \emph{Chain} shape because it has also the properties of the \emph{Single-Edge} properties and the number of its properties is easy for illustration. You can find the results of the more complex shapes at the end of this paper. The first three rows represent the properties of the \emph{Single-Edge} shape in which the system answered correctly 73 questions from 109. The next four rows show the system ability to answer some of \emph{Chain} questions of \emph{Select} query where the number of triples equal to 2 or 3 but unfortunately, there were not questions with triples more than 3 to check the effect of them on the system. The remaining rows are the questions that the system cannot deal with them at all. This is due to complexity of these question that appear in the requirement of using more keywords as \emph{limit}, \emph{offset}, \emph{not-exist}, \emph{filter} and/or \emph{graph} or using queries of \emph{Ask}.


Figure \ref{fig:gAnswerStar} shows that \emph{gAnswer} can only deal with the simplest type of \emph{Star} shape in which triples are \emph{CQ} and keywords used in the queries are \emph{select}, \emph{distinct} and \emph{and}, and the number of triples are 3. When the query category changed or the number of keywords or triples increased, the system struggle with them. An example of questions with \emph{Star} shape that \emph{gAnswer} answered it is given in Listing \ref{listing:gAnswerStar1} while another example that \emph{gAnswer} cannot answer it is given in Listing \ref{listing:gAnswerStar2}.

% \begin{scriptsize}
% \begin{minipage}{\linewidth}
% \begin{lstlisting} [language=SPARQL, label=listing:gAnswerStar1, caption=Q: Which electronics companies were founded in Beijing?]

% SELECT DISTINCT ?uri WHERE { 
%     ?uri 
%     a 
%     <http://dbpedia.org/ontology/Company> 
%     .
%     ?uri 
%     <http://dbpedia.org/ontology/industry>
%     <http://dbpedia.org/resource/Electronics> 
%     . 
%     ?uri 
%     <http://dbpedia.org/ontology/foundationPlace>
%     <http://dbpedia.org/resource/Beijing> 
%     .
% }
% \end{lstlisting}
% \end{minipage}
% \end{scriptsize}

% \begin{scriptsize}
% \begin{minipage}{\linewidth}
% \begin{lstlisting} [language=SPARQL, label=listing:gAnswerStar2, caption=Q: Which Chess players died in the same place they were born in?]
% SELECT DISTINCT ?uri WHERE {  
%     ?uri 
%     <http://www.w3.org/1999/02/22-rdf-syntax-ns#type>
%     <http://dbpedia.org/ontology/ChessPlayer>
%     .
%     ?uri
%     <http://dbpedia.org/ontology/birthPlace> 
%     ?x 
%     .
%     ?uri 
%     <http://dbpedia.org/ontology/deathPlace> 
%     ?y 
%     .  
%     FILTER (?x = ?y) 
%     . 
% }
% \end{lstlisting}
% \end{minipage}
% \end{scriptsize}










Repeating the same experiment with \emph{WDAqua-core1} \cite{diefenbach2018wdaqua} which fed by questions from \emph{QALD 9} which used to evaluate the system. Figure  \ref{fig:PR} shows the \emph{Recall} and \emph{Precision} for the different shapes. Also, \emph{Single-Edge} has the highest \emph{Recall} and \emph{Precision} with 0.271\% and 0.62\% respectively. Although \emph{gAnswer} was a little better, \emph{WDAqua-core1} has the same behaviour of dealing with the more complex questions. \emph{WDAqua-core1} cannot answer any \emph{Cycle} questions. But this observation is not reliable as it is only tested against one \emph{Cycle} question. 

Figure \ref{fig:WDAChain} and \ref{fig:WDAStar} represent the \emph{Chain} and \emph{Star} questions analyzed for \emph{WDAqua-core1} system respectively. By comparing Figure \ref{fig:WDAChain} to \ref{fig:gAnswerChain}, we can find that the majority of questions of type \emph{Chain} that  \emph{WDAqua-core1} fed by are \emph{CQ} queries with one triple and \emph{Select} and \emph{Distinct} keywords. The system answered 52 questions out o 153 questions. On the other hand, \emph{gAnswer} evaluated mostly against 177 questions of the type \emph{CQ}, triples is equal to one and keywords are \emph{Select}, \emph{Distinct} and \emph{And}. The system answered correctly 75 questions of them. When the keywords are \emph{Select}, \emph{Distinct} and \emph{And} and \emph{T=2}, \emph{gAnswer} answered 19 out of 97 questions and \emph{WDAqua-core1} answered 5 out of 24. The percentage for the two systems are approximately the same(0.2\%). The remaining properties are not (approximately) answered.

While \emph{WDAqua-core1} answered only one question of the \emph{Star} shape (see Figure \ref{fig:WDAStar}), \emph{gAnswer} answered 6 questions as shown in Figure \ref{fig:gAnswerStar}. However, there is an important observation. While \emph{gAnswer} answered questions with simple properties, the question that \emph{WDAqua-core1} answered has more complex properties. This question has a \emph{union} keyword. 

%QALD-1 F1
%Recall = 0.05714285714285714
%precision = 0.13793103448275862
%F1 = 0.0808080808080808

%QALD-6
%Recall = 0.2967289719626168
%precision = 0.5570175438596491
%F1 = 0.3871951219512195

%QALD-9 F1
%Recall = 0.33578431372549017
%precision = 0.6227272727272727
%F1 = 0.4363057324840764

     \begin{table}
        \centering
        \captionof{table}{F1 calculated based on considering the question is correctly answered if any of the returned answers is in the correct answers. F+: when all correct answers retrieved}% Add 'table' caption
        \label{table:f1}
        \setlength{\tabcolsep}{3pt} %% default is 6pt
        \begin{tabular}{llrrr}
\toprule
	System & Benchmark & F1  & F1^+  &    \\ \midrule
	%gAnswer & QALD-1 & 0.08 & - &    \\ 
	gAnswer & QALD-6 & 0.39 & - &    \\ 
	gAnswer & QALD-9 & 0.44 & - &    \\ 
	WDAqua-core1 & QALD-1 & 0.19 & 0.14 & \\
	WDAqua-core1 & QALD-6 & 0.16 & 0.12 & \\
	WDAqua-core1 & QALD-9 & 0.17 & 0.14 &    \\ 
    \bottomrule
\end{tabular}

        \end{table}

%\begin{figure}[tbp]
%  \includegraphics[width=0.85\linewidth]{WDAPR}
%  \caption{Recall and Precision Analysis for WDAqua-core1 System with respect to Queries Shapes.}
%  \label{fig:WDAPR}
%\end{figure}





\begin{figure}[tbp]
  \includegraphics[width=0.9\linewidth]{figures/WDAChain.png}
  \caption{Chain Questions Answered by WDAqua-core1 for Different Properties.}
  \label{fig:WDAChain}
\end{figure}

\begin{figure}[tbp]
  \includegraphics[width=0.9\linewidth]{figures/WDAStar.png}
  \caption{Star Questions Answered by WDAqua-core1 for Different Properties.}
  \label{fig:WDAStar}
\end{figure}





==> sections/QA_Systems.tex <==
\section{Overview of Question Answering Over Knowledge Graphs Systems}
\label{sec:qa}

\textbf{Automated Template Generation for Question Answering over Knowledge Graphs:} \\
QUINT automatically learns the question-query templates from user questions associated with their answers set. This system uses the training time to produce templates. A template is composed of 3 components namely: a query template, an utterance template, an alignment between the query and utterance templates. An utterance is defined as a message or spoken words from a person through a conversation \cite{bernsen2012designing}. During the testing time, these templates are applied to evaluate answering questions, because a template is composed by a pair between a question utterance and its answer set in the knowledge graph. The templates are dependent on standard dependency parse tree. To create a query, the training utterance is annotated by means of named entities it holds, and then follows the process of eliminating ambiguity to match these with Freebase entities. The query is expressed in the form of SPARQL style triple-pattern language. The alignment between a question and a query is built using integer linear programming. The system is divided into online and offline phase. The learning of templates is done in the offline phase; the online phase is when the user interacts with the system. QUINT uses lightweight machine, it uses basic templates to answer the complex questions formed with multiple clauses. QUINT decomposes a complex question into a set of simple sub-questions.  A ranked list of queries is attached to each sub-question. QUINT answers each simple sub-question of the set independently. Sub-questions combine the results of their queries to answer the complex question. The relationship between semantic items from the knowledge graph and a question vocabulary is performed through lexicons. A lexicon has two parts, the predicate lexicon and the type lexicon. The distance supervision \cite{Mintz2009} is applied to build lexicons. In distant supervision, when two entities are involved in a relation, any sentence carrying those two entities can represent the relation. To create the lexicons, QUINT utilized ClueWeb09-FACC1, a corpus of 500M Web pages annotated with Freebase entities. It used NER/NED \cite{DBLP:journals/corr/YangC16a} a disambiguation system resolving ambiguity with the mean of entity relationships. \\

\textbf{Critique:}\\
This system presents some limitations in the way it operates. First, it relies on the alignment information between unit of speech called utterance and query that may present errors bringing knowledge based question answering to fail in providing answers. It does not provide any mechanism to handle questions syntactic structure is invisible. QUINT involves multiple KG predicates, so that it generates empty lookups when the predicate lexicons are deficient.  The dependency parse tree accuracy is another inconvenience of this system, because some words could not be labeled properly, altering their meaning, thus queries created could be incorrect. This may fail to correspond a question to a template influencing the precision of a query. QUINT depends on (NER/NED) \cite{yang2016s}, a system for the disambiguation and recognition of entities. QUINT is not able to identify errors or mistakes from (NER/NED), which implies that it may provide false answers when there are errors. QUINT requires a precise system of recognition of the entities.

\textbf{Question Answering with Subgraph Embeddings:}\\
Bordes et al \cite{BordesCW14} introduces a model that uses a small number of hand-crafted features in a knowledge base to answer questions. It uses low-dimensional vector embeddings of words for learning purposes. Words come from entities and questions. A scoring function to learn embeddings, composed by a combination of a question and a candidate answer is employed. The higher the precision of the answer to the question, the higher the scoring function is. The answers come in three different representations related to the subgraph of the KB:  Single entity, path representation and subgraph representation.  Single entity depicts an answer as one entity. The path representation applies one or two hops from the entity in the question toward the answer entity. The subgraph representation merges the path representation and entities’ subgraph. The size of the dictionary of embeddings to be learned is doubled to increase the ways answer path could be presented to refine results. A margin-based ranking loss function is used to train the set of questions with their answers. The loss function is minimized to increase the score of combination of a question and an accurate answer, followed by gradient descent stochastic optimization.\\

\textbf{Critique:}\\
This system is limited in terms of querying because it concentrates questions and their answers on a specific knowledge base. It uses a subset of Freebase and keeps only triples that are contained in either Webquestions or ClueWeb. It also removes all entities present less than five times in Freebase. It is not suitable to extend it to other knowledge bases. The accuracy of the inference method used can be harmed when the number of candidates increases while considering all connections generated using two hops paths.\\ 
\textbf{More Accurate Question Answering on Freebase:}\\
Hannah et al focus on aqqu, a system that can automatically convert a natural-language question into a format corresponding  to a SPARQL query from a knowledge base. To achieve that, aqqu includes these components in the architecture: entity matching, candidate generation, relation matching, candidate features, ranking, and candidate pruning. The entity matching discovers all entities in the knowledge base that correspond to a fragment of a question. aqqu uses stanford [] tagger to tag questions. aqqu applies NN, NNP  tags for subsequence of a single word such as noun and proper noun. To match entities, aqqu finds all entities in the knowledge base that are corresponding to tagged nouns in the question. aqqu uses CrossWikis [], a tool to connect text strings to Wikipedia concept. For each noun s matching in the KB, a score is provided with the mean of CrossWiki which provides the probability distribution measurement to score the matching. Then, aqqu determines the popularity of the score of an entity by counting how many times an entity is cited in the ClueWeb12 [ ], a dataset containing millions of English web pages. Relying on the entity matches, aqqu can produce query candidates in three disjoint subsets, representing three templates. These three templates substitute for a query presenting a distinct form of structure, and they include practically the entire set of questions used in both Free917 and WebQuestions. To match relations, aqqu defines a set of lemmatized words from relations contained in the set of query candidates. The set of lemmatized words are compared to those from a question to know how suitable they match. Aqqu applies 4 types of matches: iteral,  derivation,  synonyms,  context. The answer type matching accomplishes a verification on the relation conducting to the answer. By summing up the types of objects in all triples, aqqu calculates the list of target types for each relation.  A candidate's feature vector is created , depending on the score. The vector feature includes the entity and N-Gram relation matching features. In N-Gram, a L2-regularized logistic regression classifier is applied to all correct candidates to be positive cases and the rest as negative cases. The feature vectors is involved in ranking query candidates. Only the top ranked query candidate is applied to produce the answer. Two ranking methods involved to find the answer:  pairwise and pointwise rankings. Pairwise ranking expresses the ranking as a binary classification problem, to predict from a pair of candidates which one is suitable to be ranked first. In Pointwise the score is processed for each candidate with the mean of the classifier L2-regularized logistic regression and random forest, then candidate are arranged based on the score.  Both methods apply logistic regression and random forest classifiers. aqqu includes a pruning technique to handle the questions when the set of query candidates is empty. The pruning eliminates evident bad candidates such as those that do not correspond to the type of answer. The pruning classifier is training with the logistic regression. 

\textbf{Critique:}\\
This system only depends on three kinds of templates. This limits the system to be extended to other knowledge bases. Also, it cannot depict structure that are compositional, and its design doesn’t allow it to handle complex questions, thus this system is suitable for simple questions. Question should start with defined patterns such as who, what, what to be handled by answer type matching. The system only works for single passage but could be challenged in the presence of union including multiple passages. The Pairwise ranking doesn't provide any mechanism to ensure if the relation that is learned could be transitive or anti-symmetric. PointWise keeps in the same class correct query  candidates  of  questions  of  different  types and difficulty. This doesn't allow to make comparison or differentiate them.\\

\textbf{Information Extraction over Structured Data: Question Answering with Freebase:}\\
Yoa et al rely on information extraction (IE) modest techniques combined with a web-scale corpus to present an automatic method for question answering. This system relies on topic graph features to select only a view of the KB that contains topics involved in the question.  The answer is extracted by examining each related node by means of hops of relations. Graph features include : question graph, Freebase topic graph and feature production. Question graph introduces dependency-based features focused on linguistic information to answer questions such as : question word, question focus, question verb, question topic. This system provides 9 common Question word such as : what, who, how. Question focus includes terms like name, question verb extracts information about verbs. Question topic assists to determine the relevant pages in Freebase. The dependency-based features allow a number of transformation on a question in question feature graph, such that all nodes and relations could be possible relevant features for the question. For each node, Freebase graph exploit both relations and properties as features, and use them to determine the answer. properties give details about the attributes of node. Additional information about alignment-based features is provided to determine how well relations are mapped to the original question. Freebase features and question features are merged using  pairwise concatenation so that the total number of features becomes large enough to apply machine learning.  Naive Bayes formula is applied to find  probability to find an optimal relation when a question of a word vector is provided. \\

\textbf{Critique:}\\
This system generates a huge number of features ,and this can affect the learning process, same time reduce the quality of the answer, such as to  provide an answer that is not respecting the correctness. Also, the great number of features can affect the computing time. Handling compositional question including relations and entities is another drawback of this system, it is missing sophisticated representation and using simple machine learning techniques. This implies per question, this system is not able  to predict multiple relations.\\

\textbf{Transforming Dependency Structures to Logical Forms for Semantic Parsing:}\\
Noticing a deficiency of a powerful type system, Siva et al present a novel approach relying on lambda calculus, to obtain logical forms of sentences by means of a transformation of dependency structure.  Lambda calculus involved in this paper depends on three base types: Individuals (Ind) brought by noun, events (Event) representing verbs and Boolean true values as functions of whole sentences. The combination of these three base types are used to represent more types such as product type (Ind X Event). Practically, this paper performs three steps to convert a dependency tree into the logical form: binarization, substitution, composition. In the binarization an s-expression is mapped to a dependency tree. An s-expression contains three expressions, with the first expression representing the dependency label, while the two last representing either a word or an s-expression. In the substitution step, a lambda expression is allocated to each word or label in the s-expression. In the composition step, the final semantic of the sentence is calculated using lambda-expression created by beta-reduction. A number of linguistic constructions are exploited such as prepositional phrases, conjunctions, relative clauses and Wh- questions (who, whom, what, when, where, why). In prepositional phrases similar s-expressions are applied to nouns and verbs. The conjunction construction is applied to a variable that is appearing in two sub-expressions and connecting them together. Relative clauses step applies a group of heuristic rules to attach annotations on the dependency parse tree, a binding variable is also attached to the sentence. Wh-questions are managed using a binding mechanism. To map the logical forms to a semantic representation for question answering, the logical forms are transformed into their analogous ungrounded graphs, then nodes and entities are mapped to Freebase subgraphs. A contract operation is applied to combine nodes connected by an edge into a unique node. To map ungrounded graphs to grounded graphs a linear learning model is used.\\

\textbf{Critique:}\\
One of the drawbacks of this system is that, it depends on a repository of manual rules, thus it uses a manual approach to pair questions and answers to learn mapping to Freebase. Another issue of this system is that it uses an external parser. To associate the intermediate representation to logical form, it necessitates a separate external ontology matching step. This system is not able to find an answer when it deals with many constraints systematically. To search some lexical information such as quantifiers or negation marker, this system necessitates much effort.\\

\textbf{Knowledge-Based Question Answering as Machine Translation:}\\
This paper presents  a work on a new unified framework that handles the two main challenges of knowledge-based question answering (KB-QA), namely:  convert natural language questions in their meaning representations, and create  meaning representations to knowledge base (KB) in order to extract answers using CYK parsing.  A QA job is considered in the same way as a translation procedure as expressed by machine translation (MT) ideas. The translation allows to create a set of formal triples-answer pairs from a specified KB and a natural language (NL) question, then evaluated by a distribution  probability. To achieve this translation process , this paper involved four tasks: search space generation, question translation,  feature design and feature weight. The first task deals with the creation of a search space. For each inserted natural question, a search space is created. From the suggested search space algorithm, for any unary span of the question, a triple set is created by means of the question translation method. The second task relies on the question translation, changes all question spans to their equivalent formal tirples. This step verifies that each span question is represented as a single-relation question. The simple-relation representation is beneficial in reducing the semantic parsing efforts. A question pattern-based translation algorithm is suggested in order to create triples. Another goal of this step is to provide  a  group of disambiguated entities from the KB. An algorithm on relation expression based question translation is provided to run when the algorithm question predicate based method is unsuccessfully achieved. For questions that produce multiple constraints a dependency tree-based method is suggested, this method fragment the question into a group of sub-questions by means of syntax-based patterns. The final answer is the intersection of the answers of all sub-questions. The third task presents a number of features sets that are applied to the distribution probability that scores formal triples-answers pairs. Features such as : to  determine the total number of original questions works, number of the spans transformed into formal triples, number of triples with predicates that are not null. In the last task, a minimum error training is introduced to adjust the weights of the feature, the goal is to attempt to find a feature weight that is able to reduce errors of top-1 answer of questions in the set of question-answer pairs. \\

\textbf{Critique:}\\
This system cannot automatically retrieve question patterns. also to define features, it uses a manual approach. Moreover, this system does rely on simple semantic constraints to answer questions, thus this system cannot handle complex questions.


==> sections/Results_ALL.tex <==

\clearpage% Flush earlier floats (otherwise order might not be correct)

    \begin{landscape}% Landscape page
    \begin{scriptsize}
    \centering
          \begin{table}
           
        \setlength{\tabcolsep}{3pt} %% default is 6pt
        \begin{tabular}{|l|ll|ll|ll|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
	 & \multicolumn{2}{l}{QALD 1}  & \multicolumn{2}{l}{QALD 2}  & \multicolumn{2}{l}{QALD 3}  & \multicolumn{2}{l}{QALD 4}  & \multicolumn{2}{l}{QALD 5}  & \multicolumn{2}{l}{QALD 6}  & \multicolumn{2}{l}{QALD 7}  & \multicolumn{2}{l}{QALD 8}  & \multicolumn{2}{l}{QALD 9}  & \multicolumn{2}{l}{QALD ALL}  & \multicolumn{2}{l}{LC-QUAD}  & \multicolumn{2}{l}{FREEBASE}  \\ \hline
	 & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% \\ \hline
	Select 
	& 165 & 91.16 
	& 264 & 90.1 
	& 340 & 91.15 
	& 237 & 91.51 
	& 289 & 92.04 
	& 386 & 92.79 
	& 390 & 88.04 
	& 280 & 89.17 & 358 & 90.63 & 915 & 91.87 & 4630 & 92.64 & 5272 & 100 \\ 
	Ask & 16 & 8.84 & 29 & 9.9 & 33 & 8.85 & 22 & 8.49 & 25 & 7.96 & 30 & 7.21 & 53 & 11.96 & 34 & 10.83 & 37 & 9.37 & 81 & 8.13 & 368 & 7.36 & 0 & 0 \\ \hline
	Distinct 
	& 65 & 35.1 
	& 216 & 73.72 
	& 301 & 80.7 
	& 226 & 87.26 
	& 271 & 86.31 
	& 360 & 86.54 
	& 342 & 77.2 
	& 213 & 67.83 
	& 301 & 76.2 
	
	
	
	& 743 & 74.6 & 4630 & 92.64 & 106 & 2.01 \\ 
	Limit 
	& 7 & 3.87 
	& 12 & 4.1 
	& 15 & 4.02 
	& 20 & 7.72 
	& 28 & 8.92 
	& 34 & 8.17 
	& 33 & 7.45 
	& 35 & 11.15 
	& 38 & 9.62 
	
	
	
	& 63 & 6.33 & 0 & 0 & 8 & 0.15 \\ 
	
	Offset 
	& 0 & 0 
	& 5 & 1.71 
	& 7 & 1.88 
	& 15 & 5.79 
	& 26 & 8.28 
	& 32 & 7.69 
	& 19 & 4.29 
	& 17 & 5.41 
	& 24 & 6.08 
	

	
	
	& 38 & 3.82 & 0 & 0 & 0 & 0 \\ 
	
	Order By 
	& 7 & 3.87 
	& 12 & 4.1 
	& 15 & 4.02 
	& 20 & 7.72 
	& 28 & 8.92 
	& 34 & 8.17 
	& 33 & 7.45 
	& 30 & 9.55 
	& 35 & 8.86 
	& 58 & 5.82 
	
	& 0 & 0 & 8 & 0.15 \\ \hline
	
	Filter 
	& 77 & 42.54 
	& 157 & 53.58 
	& 49 & 13.14 
	& 29 & 11.2 
	& 27 & 8.6 
	& 28 & 6.73 
	& 49 & 11.06 
	& 14 & 4.46 
	& 29 & 7.34 
	
		
	
	& 132 & 13.25 & 1 & 0.02 & 5193 & 98.5 \\ 
	
	And (.) 
	& 83 & 45.86 
	& 121 & 41.30 
	& 124 & 33.24 
	& 50 & 19.31 
	& 54 & 17.20 
	& 73 & 7.55 
	& 68 & 5.35 
	& 48 & 15.29 
	& 57 & 14.43 
	
	& 243 & 24.40 & 1606 & 32.13 & 1899 & 36.02 \\
	
	Union 
	& 13 & 7.18 
	& 19 & 6.48 
	& 20 & 5.36 
	& 23 & 8.88 
	& 32 & 10.19 
	& 34 & 8.17 
	& 23 & 5.19 
	& 6 & 1.91 
	& 27 & 6.84 
	
	& 61 & 6.12 & 20 & 0.4 & 31 & 0.59 \\
	
	Opt 
	& 64 & 35.36 
	& 135 & 46.08 
	& 3 & 0.8 
	& 1 & 0.39 
	& 1 & 0.32 
	& 1 & 0.24 
	& 27 & 6.09 
	& 1 & 0.32 
	& 1 & 0.25 
	& 52 & 5.22 
	
	There is a large variation between QALD-1 and other QALDs with respect to the Distinct keyword where only 35\% of QALD-1 queries use Distinct keyword, the other QALDs have ranges between 73\% to 87\% queries with this keyword. The Limit keyword steadily increased from 7 times in QALD-1 to 38 times in QALD-9 with unstable percentages from 3.8\% to 11.2\%. The offset keyword is rarely used in QALD-1 to 3 and has higher ration in other QALDs (from 5\% to 8\%). The Filter and Opt keywords have (42.5\% and 53.6\%) and (35.4\% and 46.1\%) in QALD-1 and QALD-2 respectively while this ration does not exceed (11\%) and (6\%) in other QALDs.
	
	& 3 & 0.06 & 0 & 0 \\
	Not Exists & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 0.48 & 2 & 0.45 & 2 & 0.64 & 0 & 0 & 2 & 0.2 & 0 & 0 & 2 & 0.04 \\
	Minus & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 0.77 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 0.2 & 0 & 0 & 5 & 0.09 \\
	
	Aggregators 
	& 18 & 9.94 
	& 32 & 10.92 
	& 39 & 10.46 
	& 15 & 5.79 
	& 18 & 5.73 
	& 25 & 6.01 
	& 25 & 5.64 
	& 16 & 5.1 
	
	
	& 20 & 5.06 & 78 & 7.83 & 658 & 13.17 & 710 & 13.47 \\ Group-By & 18 & 9.94 & 32 & 10.92 & 39 & 10.46 & 15 & 5.79 & 18 & 5.73 & 25 & 6.01 & 25 & 5.64 & 16 & 5.1 & 20 & 5.06 & 78 & 7.83 & 658 & 13.17 & 710 & 13.47 \\ 
	
	Having 
	& 1 & 0.55 
	& 6 & 2.05 
	& 8 & 2.14 
	& 2 & 0.77 
	& 2 & 0.64 
	& 3 & 0.72 
	& 3 & 0.68 
	& 1 & 0.32 
	& 3 & 0.76 
	
	& 13 & 1.31 & 0 & 0 & 0 & 0 \\ \hline
\end{tabular}
\captionof{table}{Keyword count in queries for each benchmark. A\# is the absolute value and R\% is the relative value.}% Add 'table' caption

          \label{table:keywordsALL}
        \end{table}
        
        \centering
        \begin{table}
        \setlength{\tabcolsep}{1.5pt} %% default is 6pt
        \begin{tabular}{|l|ll|ll|ll|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
	 & \multicolumn{2}{l}{QALD 1}  & \multicolumn{2}{l}{QALD 2}  & \multicolumn{2}{l}{QALD 3}  & \multicolumn{2}{l}{QALD 4}  & \multicolumn{2}{l}{QALD 5}  & \multicolumn{2}{l}{QALD 6}  & \multicolumn{2}{l}{QALD 7}  & \multicolumn{2}{l}{QALD 8}  & \multicolumn{2}{l}{QALD 9}  & \multicolumn{2}{l}{QALD ALL}  & \multicolumn{2}{l}{LC-QUAD}  & \multicolumn{2}{l}{FREEBASE}  \\ \hline
& A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% \\ \hline
	none & 36 & 19.89 & 50 & 17.06 & 216 & 57.91 & 182 & 70.27 & 228 & 72.61 & 306 & 73.56 & 328 & 74.04 & 256 & 81.53 & 304 & 76.96 & 636 & 63.86 & 3351 & 67.05 & 19 & 0.36 \\ 
	F & 7 & 3.87 & 6 & 2.05 & 16 & 4.29 & 11 & 4.25 & 10 & 3.18 & 12 & 2.88 & 6 & 1.35 & 3 & 0.96 & 11 & 2.78 & 28 & 2.81 & 1 & 0.02 & 3253 & 61.7 \\ 
	A & 65 & 35.91 & 86 & 29.35 & 96 & 25.74 & 31 & 11.97 & 34 & 10.83 & 54 & 12.98 & 48 & 10.84 & 36 & 11.46 & 39 & 9.87 & 186 & 18.67 & 1584 & 31.69 & 38 & 0.72 \\ 
	A, F & 8 & 4.42 & 15 & 5.12 & 22 & 5.9 & 10 & 3.86 & 8 & 2.55 & 7 & 1.68 & 15 & 3.39 & 10 & 3.18 & 10 & 2.53 & 42 & 4.22 & 0 & 0 & 1808 & 34.29 \\ \hline \hline
	CPF Subtotal & 116 & 64.09 & 157 & 53.58 & 350 & 93.83 & 234 & 90.35 & 280 & 89.17 & 379 & 91.11 & 397 & 89.62 & 305 & 97.13 & 364 & 92.15 & 892 & 89.56 & 4936 & 98.76 & 5118 & 97.08 \\ \hline \hline
	O & 2 & 1.1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0.1 & 1 & 0.02 & 0 & 0 \\ 
	O, F & 41 & 22.65 & 100 & 34.13 & 2 & 0.54 & 1 & 0.39 & 1 & 0.32 & 1 & 0.24 & 22 & 4.97 & 1 & 0.32 & 1 & 0.25 & 37 & 3.71 & 0 & 0 & 0 & 0 \\ 
	A, O & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 0.04 & 0 & 0 \\ 
	A, O, F & 9 & 4.97 & 17 & 5.8 & 1 & 0.27 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 0.2 & 0 & 0 & 0 & 0 \\ \hline \hline
	CPF + O & +52 & +28.73 & +117 & +39.93 & +3 & +0.8 & +1 & +0.39 & +1 & +0.32 & +1 & +0.24 & +22 & +4.97 & +1 & +0.32 & +1 & +0.25 & +40 & +4.02 & +3 & +0.06 & +0 & +0 \\ \hline \hline
	G & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0.39 & 1 & 0.32 & 2 & 0.48 & 1 & 0.23 & 2 & 0.64 & 3 & 0.76 & 3 & 0.3 & 26 & 0.52 & 0 & 0 \\ \hline \hline
	CPF + G & +0 & +0 & +0 & +0 & +0 & +0 & +1 & +0.39 & +1 & +0.32 & +2 & +0.48 & +1 & +0.23 & +2 & +0.64 & +3 & +0.76 & +3 & +0.3 & +26 & +0.52 & +0 & +0 \\ \hline \hline
	U & 1 & 0.55 & 0 & 0 & 8 & 2.14 & 8 & 3.09 & 13 & 4.14 & 15 & 3.61 & 12 & 2.71 & 4 & 1.27 & 13 & 3.29 & 27 & 2.71 & 13 & 0.26 & 12 & 0.23 \\ 
	U, F & 0 & 0 & 1 & 0.34 & 7 & 1.88 & 6 & 2.32 & 7 & 2.23 & 7 & 1.68 & 1 & 0.23 & 0 & 0 & 6 & 1.52 & 9 & 0.9 & 0 & 0 & 0 & 0 \\ 
	A, U & 0 & 0 & 0 & 0 & 4 & 1.07 & 8 & 3.09 & 11 & 3.5 & 11 & 2.64 & 5 & 1.13 & 2 & 0.64 & 7 & 1.77 & 11 & 1.1 & 7 & 0.144 & 8 & 0.15 \\ 
	A, U, F & 0 & 0 & 0 & 0 & 1 & 0.27 & 1 & 0.39 & 1 & 0.32 & 1 & 0.24 & 0 & 0 & 0 & 0 & 1 & 0.25 & 2 & 0.2 & 0 & 0 & 11 & 0.21 \\ \hline \hline
	CPF + U & +1 & +0.554 & +1 & +0.34 & +20 & +5.36 & +23 & +8.884 & +32 & +10.19 & +34 & +8.17 & +18 & +4.06 & +6 & +1.91 & +27 & +6.84 & +49 & +4.92 & +20 & +0.4 & +31 & +0.59 \\ \hline

\end{tabular}
\captionof{table}{Sets of operators used in queries: Filter (F), And (A), Opt (O), Graph (G), and Union (U) for each dataset}% Add 'table' caption
        \label{table:operatorsALL}
        \end{table}
        
        
        
    \end{scriptsize}
    \end{landscape}
\clearpage% Flush page









\clearpage% Flush earlier floats (otherwise

\begin{longtable}
\label{table:categories}
\centering
\begin{tiny}
\begin{tabular}{lllllll}
\hline \hline
& & \multicolumn{2} {c}{QALD 1} & & & \\
\hline \hline
            & \textit{CQ}        &            &\textit{CQ\textsubscript{F}}        &            &\textit{CQ\textsubscript{OF}}           &             \\ \hline
Shape       & \#Qs & Re\% & \#Qs & Re\% & \#Qs & Re\%  \\ \hline
Single Edge & 12    & 11.88\%    & 12      & 10.34\%    & 12      & 7.14\% \\
Chain       & 44          & 43.56\%    &       51      & 43.97\%    & 66      & 39.29\% \\ 
Chain Set   & 44       & 43.56\%    &    52      & 44.83\%    & 68      & 40.48\% \\
Star        & 42           & 41.58\%    &        49      & 42.24\%    & 81      & 48.21\% \\
Tree        & 100           & 99.01\%    &        114      & 98.28\%    & 162      & 96.43\% \\
Forest      & 100         & 99.01\%    &      115      & 99.14\%    & 167      & 99.40\% \\ \hline
Cycle       & 0          & 0.00\%    &       0      & 0.00\%    & 0      & 0.00\% \\
Flower      & 101         & 100.00\%    &      115      & 99.14\%    & 164      & 97.62\% \\
Flower-Set  & 101      & 100.00\%    &   115      & 99.14\%    & 164      & 97.62\% \\ \hline
Total       & 101      & 100.0\%    & 116      & 100.0\%    & 168      & 100.0\%
\end{tabular}

\begin{tabular}{lllllll}
\hline \hline
& & \multicolumn{2} {c}{QALD 2} & & & \\
\hline \hline
            & \textit{CQ}        &            &\textit{CQ\textsubscript{F}}        &            &\textit{CQ\textsubscript{OF}}           &             \\ \hline
Shape       & \#Qs & Re\% & \#Qs & Re\% & \#Qs & Re\%  \\ \hline
Single Edge & 28    & 20.59\%    & 29      & 18.47\%    & 29      & 10.58\% \\
Chain       & 62          & 45.59\%    &       69      & 43.95\%    & 128      & 46.72\% \\ 
Chain Set   & 62       & 45.59\%    &    69      & 43.95\%    & 128      & 46.72\% \\
Star        & 48           & 35.29\%    &        54      & 34.39\%    & 106      & 38.69\% \\
Tree        & 136           & 100.00\%    &        151      & 96.18\%    & 264      & 96.35\% \\
Forest      & 136         & 100.00\%    &      154      & 98.09\%    & 271      & 98.91\% \\ \hline
Cycle       & 0          & 0.00\%    &       0      & 0.00\%    & 0      & 0.00\% \\
Flower      & 136         & 100.00\%    &      152      & 96.82\%    & 265      & 96.72\% \\
Flower-Set  & 136      & 100.00\%    &   152      & 96.82\%    & 265      & 96.72\% \\ \hline
Total       & 136      & 100.0\%    & 157      & 100.0\%    & 274      & 100.0\%
\end{tabular}

\begin{tabular}{lllllll}
\hline \hline
& & \multicolumn{2} {c}{QALD 3} & & & \\
\hline \hline
            & \textit{CQ}        &            &\textit{CQ\textsubscript{F}}        &            &\textit{CQ\textsubscript{OF}}           &             \\ \hline
Shape       & \#Qs & Re\% & \#Qs & Re\% & \#Qs & Re\%  \\ \hline
Single Edge & 124    & 39.74\%    & 124      & 35.43\%    & 126      & 35.69\% \\
Chain       & 228          & 73.08\%    &       247      & 70.57\%    & 249      & 70.54\% \\ 
Chain Set   & 228       & 73.08\%    &    251      & 71.71\%    & 253      & 71.67\% \\
Star        & 55           & 17.63\%    &        63      & 18.00\%    & 64      & 18.13\% \\
Tree        & 311           & 99.68\%    &        339      & 96.86\%    & 342      & 96.88\% \\
Forest      & 312         & 100.00\%    &      347      & 99.14\%    & 350      & 99.15\% \\ \hline
Cycle       & 1          & 0.32\%    &       1      & 0.29\%    & 1      & 0.28\% \\
Flower      & 312         & 100.00\%    &      342      & 97.71\%    & 345      & 97.73\% \\
Flower-Set  & 312      & 100.00\%    &   342      & 97.71\%    & 345      & 97.73\% \\ \hline
Total       & 312      & 100.0\%    & 350      & 100.0\%    & 353      & 100.0\%
\end{tabular}

\begin{tabular}{lllllll}
\hline \hline
& & \multicolumn{2} {c}{QALD 4} & & & \\
\hline \hline
            & \textit{CQ}        &            &\textit{CQ\textsubscript{F}}        &            &\textit{CQ\textsubscript{OF}}           &             \\ \hline
Shape       & \#Qs & Re\% & \#Qs & Re\% & \#Qs & Re\%  \\ \hline
Single Edge & 110    & 51.64\%    & 110      & 47.01\%    & 111      & 47.23\% \\
Chain       & 188          & 88.26\%    &       199      & 85.04\%    & 200      & 85.11\% \\ 
Chain Set   & 188       & 88.26\%    &    201      & 85.90\%    & 202      & 85.96\% \\
Star        & 15           & 7.04\%    &        19      & 8.12\%    & 19      & 8.09\% \\
Tree        & 212           & 99.53\%    &        228      & 97.44\%    & 229      & 97.45\% \\
Forest      & 213         & 100.00\%    &      234      & 100.00\%    & 235      & 100.00\% \\ \hline
Cycle       & 1          & 0.47\%    &       1      & 0.43\%    & 1      & 0.43\% \\
Flower      & 213         & 100.00\%    &      229      & 97.86\%    & 230      & 97.87\% \\
Flower-Set  & 213      & 100.00\%    &   229      & 97.86\%    & 230      & 97.87\% \\ \hline
Total       & 213      & 100.0\%    & 234      & 100.0\%    & 235      & 100.0\%
\end{tabular}

\begin{tabular}{lllllll}
\hline \hline
& & \multicolumn{2} {c}{QALD 5} & & & \\
\hline \hline
            & \textit{CQ}        &            &\textit{CQ\textsubscript{F}}        &            &\textit{CQ\textsubscript{OF}}           &             \\ \hline
Shape       & \#Qs & Re\% & \#Qs & Re\% & \#Qs & Re\%  \\ \hline
Single Edge & 135    & 51.53\%    & 135      & 48.21\%    & 136      & 48.40\% \\
Chain       & 231          & 88.17\%    &       238      & 85.00\%    & 239      & 85.05\% \\ 
Chain Set   & 231       & 88.17\%    &    240      & 85.71\%    & 241      & 85.77\% \\
Star        & 21           & 8.02\%    &        27      & 9.64\%    & 27      & 9.61\% \\
Tree        & 260           & 99.24\%    &        273      & 97.50\%    & 274      & 97.51\% \\
Forest      & 262         & 100.00\%    &      280      & 100.00\%    & 281      & 100.00\% \\ \hline
Cycle       & 1          & 0.38\%    &       1      & 0.36\%    & 1      & 0.36\% \\
Flower      & 261         & 99.62\%    &      274      & 97.86\%    & 275      & 97.86\% \\
Flower-Set  & 261      & 99.62\%    &   274      & 97.86\%    & 275      & 97.86\% \\ \hline
Total       & 262      & 100.0\%    & 280      & 100.0\%    & 281      & 100.0\%
\end{tabular}

\begin{tabular}{lllllll}
\hline \hline
& & \multicolumn{2} {c}{QALD 6} & & & \\
\hline \hline
            & \textit{CQ}        &            &\textit{CQ\textsubscript{F}}        &            &\textit{CQ\textsubscript{OF}}           &             \\ \hline
Shape       & \#Qs & Re\% & \#Qs & Re\% & \#Qs & Re\%  \\ \hline
Single Edge & 200    & 55.56\%    & 201      & 53.03\%    & 202      & 53.16\% \\
Chain       & 329          & 91.39\%    &       337      & 88.92\%    & 338      & 88.95\% \\ 
Chain Set   & 329       & 91.39\%    &    339      & 89.45\%    & 340      & 89.47\% \\
Star        & 28           & 7.78\%    &        34      & 8.97\%    & 34      & 8.95\% \\
Tree        & 359           & 99.72\%    &        373      & 98.42\%    & 374      & 98.42\% \\
Forest      & 360         & 100.00\%    &      379      & 100.00\%    & 380      & 100.00\% \\ \hline
Cycle       & 1          & 0.28\%    &       1      & 0.26\%    & 1      & 0.26\% \\
Flower      & 360         & 100.00\%    &      374      & 98.68\%    & 375      & 98.68\% \\
Flower-Set  & 360      & 100.00\%    &   374      & 98.68\%    & 375      & 98.68\% \\ \hline
Total       & 360      & 100.0\%    & 379      & 100.0\%    & 380      & 100.0\%
\end{tabular}

\begin{tabular}{lllllll}
\hline \hline
& & \multicolumn{2} {c}{QALD 7} & & & \\
\hline \hline
            & \textit{CQ}        &            &\textit{CQ\textsubscript{F}}        &            &\textit{CQ\textsubscript{OF}}           &             \\ \hline
Shape       & \#Qs & Re\% & \#Qs & Re\% & \#Qs & Re\%  \\ \hline
Single Edge & 238    & 63.30\%    & 238      & 59.95\%    & 240      & 57.28\% \\
Chain       & 339          & 90.16\%    &       345      & 86.90\%    & 365      & 87.11\% \\ 
Chain Set   & 340       & 90.43\%    &    350      & 88.16\%    & 370      & 88.31\% \\
Star        & 35           & 9.31\%    &        41      & 10.33\%    & 43      & 10.26\% \\
Tree        & 375           & 99.73\%    &        387      & 97.48\%    & 409      & 97.61\% \\
Forest      & 376         & 100.00\%    &      397      & 100.00\%    & 419      & 100.00\% \\ \hline
Cycle       & 0          & 0.00\%    &       0      & 0.00\%    & 0      & 0.00\% \\
Flower      & 375         & 99.73\%    &      387      & 97.48\%    & 409      & 97.61\% \\
Flower-Set  & 375      & 99.73\%    &   387      & 97.48\%    & 409      & 97.61\% \\ \hline
Total       & 376      & 100.0\%    & 397      & 100.0\%    & 419      & 100.0\%
\end{tabular}

\begin{tabular}{lllllll}
\hline \hline
& & \multicolumn{2} {c}{QALD 8} & & & \\
\hline \hline
            & \textit{CQ}        &            &\textit{CQ\textsubscript{F}}        &            &\textit{CQ\textsubscript{OF}}           &             \\ \hline
Shape       & \#Qs & Re\% & \#Qs & Re\% & \#Qs & Re\%  \\ \hline
Single Edge & 195    & 66.78\%    & 195      & 63.93\%    & 196      & 64.05\% \\
Chain       & 266          & 91.10\%    &       272      & 89.18\%    & 273      & 89.22\% \\ 
Chain Set   & 266       & 91.10\%    &    273      & 89.51\%    & 274      & 89.54\% \\
Star        & 25           & 8.56\%    &        28      & 9.18\%    & 28      & 9.15\% \\
Tree        & 292           & 100.00\%    &        301      & 98.69\%    & 302      & 98.69\% \\
Forest      & 292         & 100.00\%    &      305      & 100.00\%    & 306      & 100.00\% \\ \hline
Cycle       & 0          & 0.00\%    &       0      & 0.00\%    & 0      & 0.00\% \\
Flower      & 292         & 100.00\%    &      301      & 98.69\%    & 302      & 98.69\% \\
Flower-Set  & 292      & 100.00\%    &   301      & 98.69\%    & 302      & 98.69\% \\ \hline
Total       & 292      & 100.0\%    & 305      & 100.0\%    & 306      & 100.0\%
\end{tabular}

\begin{tabular}{lllllll}
\hline \hline
& & \multicolumn{2} {c}{QALD 9} & & & \\
\hline \hline
            & \textit{CQ}        &            &\textit{CQ\textsubscript{F}}        &            &\textit{CQ\textsubscript{OF}}           &             \\ \hline
Shape       & \#Qs & Re\% & \#Qs & Re\% & \#Qs & Re\%  \\ \hline
Single Edge & 207    & 60.35\%    & 207      & 56.87\%    & 208      & 56.99\% \\
Chain       & 314          & 91.55\%    &       325      & 89.29\%    & 326      & 89.32\% \\ 
Chain Set   & 314       & 91.55\%    &    326      & 89.56\%    & 327      & 89.59\% \\
Star        & 27           & 7.87\%    &        32      & 8.79\%    & 32      & 8.77\% \\
Tree        & 342           & 99.71\%    &        358      & 98.35\%    & 359      & 98.36\% \\
Forest      & 343         & 100.00\%    &      364      & 100.00\%    & 365      & 100.00\% \\ \hline
Cycle       & 1          & 0.29\%    &       1      & 0.27\%    & 1      & 0.27\% \\
Flower      & 343         & 100.00\%    &      359      & 98.63\%    & 360      & 98.63\% \\
Flower-Set  & 343      & 100.00\%    &   359      & 98.63\%    & 360      & 98.63\% \\ \hline
Total       & 343      & 100.0\%    & 364      & 100.0\%    & 365      & 100.0\%
\end{tabular}

\begin{tabular}{lllllll}
\hline \hline
& & \multicolumn{2} {c}{QALD ALL} & & & \\
\hline \hline
            & \textit{CQ}        &            &\textit{CQ\textsubscript{F}}        &            &\textit{CQ\textsubscript{OF}}           &             \\ \hline
Shape       & \#Qs & Re\% & \#Qs & Re\% & \#Qs & Re\%  \\ \hline
Single Edge & 404    & 49.15\%    & 405      & 45.40\%    & 408      & 43.78\% \\
Chain       & 666          & 81.02\%    &       698      & 78.25\%    & 725      & 77.79\% \\ 
Chain Set   & 667       & 81.14\%    &    705      & 79.04\%    & 732      & 78.54\% \\
Star        & 118           & 14.36\%    &        137      & 15.36\%    & 150      & 16.09\% \\
Tree        & 820           & 99.76\%    &        873      & 97.87\%    & 913      & 97.96\% \\
Forest      & 822         & 100.00\%    &      888      & 99.55\%    & 928      & 99.57\% \\ \hline
Cycle       & 1          & 0.12\%    &       1      & 0.11\%    & 1      & 0.11\% \\
Flower      & 821         & 99.88\%    &      876      & 98.21\%    & 916      & 98.28\% \\
Flower-Set  & 821      & 99.88\%    &   876      & 98.21\%    & 916      & 98.28\% \\ \hline
Total       & 822      & 100.0\%    & 892      & 100.0\%    & 932      & 100.0\%
\end{tabular}

\begin{tabular}{lllllll}
\hline \hline
& & \multicolumn{2} {c}{LC-QUAD} & & & \\
\hline \hline
            & \textit{CQ}        &            &\textit{CQ\textsubscript{F}}        &            &\textit{CQ\textsubscript{OF}}           &             \\ \hline
Shape       & \#Qs & Re\% & \#Qs & Re\% & \#Qs & Re\%  \\ \hline
Single Edge & 1259    & 25.50\%    & 1259      & 25.49\%    & 1259      & 25.49\% \\
Chain       & 3128          & 63.35\%    &       3128      & 63.33\%    & 3128      & 63.33\% \\ 
Chain Set   & 3128       & 63.35\%    &    3128      & 63.33\%    & 3128      & 63.33\% \\
Star        & 1160           & 23.49\%    &        1161      & 23.51\%    & 1161      & 23.51\% \\
Tree        & 4938           & 100.00\%    &        4939      & 100.00\%    & 4939      & 100.00\% \\
Forest      & 4938         & 100.00\%    &      4939      & 100.00\%    & 4939      & 100.00\% \\ \hline
Cycle       & 0          & 0.00\%    &       0      & 0.00\%    & 0      & 0.00\% \\
Flower      & 4938         & 100.00\%    &      4939      & 100.00\%    & 4939      & 100.00\% \\
Flower-Set  & 4938      & 100.00\%    &   4939      & 100.00\%    & 4939      & 100.00\% \\ \hline
Total       & 4938      & 100.0\%    & 4939      & 100.0\%    & 4939      & 100.0\%
\end{tabular}

\begin{tabular}{lllllll}
\hline \hline
& & \multicolumn{2} {c}{FREEBASE} & & & \\
\hline \hline
            & \textit{CQ}        &            &\textit{CQ\textsubscript{F}}        &            &\textit{CQ\textsubscript{OF}}           &             \\ \hline
Shape       & \#Qs & Re\% & \#Qs & Re\% & \#Qs & Re\%  \\ \hline
Single Edge & 7    & 12.28\%    & 8      & 0.16\%    & 8      & 0.16\% \\
Chain       & 37          & 64.91\%    &       41      & 0.80\%    & 41      & 0.80\% \\ 
Chain Set   & 37       & 64.91\%    &    41      & 0.80\%    & 41      & 0.80\% \\
Star        & 20           & 35.09\%    &        28      & 0.55\%    & 28      & 0.55\% \\
Tree        & 57           & 100.00\%    &        5116      & 99.96\%    & 5116      & 99.96\% \\
Forest      & 57         & 100.00\%    &      5118      & 100.00\%    & 5118      & 100.00\% \\ \hline
Cycle       & 0          & 0.00\%    &       0      & 0.00\%    & 0      & 0.00\% \\
Flower      & 57         & 100.00\%    &      5118      & 100.00\%    & 5118      & 100.00\% \\
Flower-Set  & 57      & 100.00\%    &   5118      & 100.00\%    & 5118      & 100.00\% \\ \hline
Total       & 57      & 100.0\%    & 5118      & 100.0\%    & 5118      & 100.0\%
\end{tabular}
\end{tiny}
\captionof{table}{Cumulative shape analysis of \textit{CQ}, \textit{CQ\textsubscript{F}}, \textit{CQ\textsubscript{OF}} across all logs.}
\label{table:shapes_}
\end{longtable}



 order might not be correct)

    \begin{landscape}% Landscape page
    \begin{scriptsize}
          \begin{table}
           \centering
           
        \setlength{\tabcolsep}{3pt} %% default is 6pt
        \begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
	 & \multicolumn{2}{c}{\textbf{QALD 1}}  & \multicolumn{2}{c}{\textbf{QALD 2}}  & \multicolumn{2}{c}{\textbf{QALD 3}}  & \multicolumn{2}{c}{\textbf{QALD 4}}  & \multicolumn{2}{c}{\textbf{QALD 5}}  & \multicolumn{2}{c}{\textbf{QALD 6}}  & \multicolumn{2}{c}{\textbf{QALD 7}}  & \multicolumn{2}{c}{\textbf{QALD 8}}  & \multicolumn{2}{c}{\textbf{QALD 9}}  & \multicolumn{2}{c}{\textbf{QALD}}  & \multicolumn{2}{c}{\textbf{LC-QUAD}}  & \multicolumn{2}{c}{\textbf{Web}} & \multicolumn{2}{c}{\textbf{Graph}}  \\ \midrule
	 & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% & A\# & R\% \\ \midrule
	Wh-Questions & 124 & 62.3 & 187 & 54.3 & 220 & 55.4 & 201 & 62.6 & 200 & 59.9 & 273 & 63.3 & 347 & 65.5 & 207 & 65.7 & 255 & 62.5 & 723 & 62.0 & 42077 & 89.0 & 5789 & 99.6 & 3166 & 61.3 \\ 
	How-Questions & 21 & 10.6 & 44 & 12.8 & 53 & 13.3 & 25 & 7.8 & 35 & 10.5 & 45 & 10.4 & 61 & 11.5 & 41 & 13.0 & 44 & 10.8 & 147 & 12.6 & 594 & 1.3 & 21 & 0.4 & 479 & 9.3 \\
	Yes/No Questions & 19 & 9.5 & 34 & 9.9 & 36 & 9.1 & 24 & 7.5 & 26 & 7.8 & 30 & 7.0 & 55 & 10.4 & 33 & 10.5 & 37 & 9.1 & 89 & 7.6 & 990 & 2.1 & 0 & 0.0 & 7 & 0.1 \\ 
	Requests & 35 & 17.6 & 78 & 22.7 & 87 & 21.9 & 68 & 21.2 & 71 & 21.2 & 81 & 18.8 & 59 & 11.1 & 34 & 10.8 & 72 & 17.6 & 197 & 16.9 & 2661 & 5.6 & 0 & 0.0 & 513 & 9.9 \\ 
	Topicalized Questions & 0 & 0 & 1 & 0.3 & 1 & 0.3 & 3 & 0.9 & 2 & 0.6 & 2 & 0.5 & 8 & 1.5 & 0 & 0 & 0 & 0 & 11 & 0.9 & 951 & 2.0 & 0 & 0.0 & 1001 & 19.4 \\ \bottomrule
\end{tabular}
\captionof{table}{Question count by type for each benchmark. A\# is the absolute value and R\% is the relative value.}% Add 'table' caption
          \label{table:type}
        \end{table}
        
        \begin{table}
        \centering
        
        \setlength{\tabcolsep}{3pt} %% default is 6pt
        \begin{tabular}{lrrrrrrrrrrrrr}
\toprule
	 & \textbf{QALD 1}  & \textbf{QALD 2}  & \textbf{QALD 3}  & \textbf{QALD 4}  & \textbf{QALD 5}  & \textbf{QALD 6}  & \textbf{QALD 7}  & \textbf{QALD 8}  & \textbf{QALD 9} & \textbf{QALD}  & \textbf{LC-QUAD}  & \textbf{Web} & \textbf{Graph}  \\ \midrule
	What & 13 & 21 & 29 & 34 & 37 & 60 & 62 & 57 & 55 & 126 & 25221 & 3212 & 1705 \\ 
	When & 19 & 22 & 27 & 10 & 12 & 18 & 27 & 15 & 14 & 70 & 0 & 239 & 3 \\
	Where & 1 & 2 & 2 & 3 & 6 & 10 & 12 & 8 & 12 & 22 & 4668 & 1078 & 56 \\ 
	Which & 63 & 92 & 101 & 115 & 92 & 112 & 141 & 66 & 105 & 318 & 6247 & 105 & 942 \\ 
	Who, whose, whom & 28 & 50 & 61 & 39 & 53 & 73 & 105 & 61 & 69 & 187 & 5918 & 1155 & 453 \\ \bottomrule
\end{tabular}
\captionof{table}{Wh-question count for each benchmark}% Add 'table' caption
          \label{table:specwh}
        \end{table}
        
        \begin{table}
        \centering
        
        \setlength{\tabcolsep}{3pt} %% default is 6pt
        \begin{tabular}{lrrrrrrrrrrrrr}
\toprule
	 & \textbf{QALD 1}  & \textbf{QALD 2}  & \textbf{QALD 3}  & \textbf{QALD 4}  & \textbf{QALD 5}  & \textbf{QALD 6}  & \textbf{QALD 7}  & \textbf{QALD 8}  & \textbf{QALD 9} & \textbf{QALD}  & \textbf{LC-QUAD}  & \textbf{Web} & \textbf{Graph}  \\ \midrule
	Cluster 1 & 9 & 13 & 11 & 20 & 10 & 9 & 19 & 10 & 11 & 16 & 14 & 3 & 32 \\ 
	Cluster 2 & 54 & 52 & 52 & 48 & 56 & 57 & 50 & 54 & 56 & 52 & 41 & 64 & 30 \\
	Cluster 3 & 37 & 35 & 37 & 32 & 34 & 34 & 31 & 36 & 33 & 32 & 45 & 33 & 38 \\ \bottomrule
\end{tabular}
\captionof{table}{Question distribution (\%) clustered based on UPOS for each benchmark}% Add 'table' caption
          \label{table:upos}
        \end{table}
        
        \begin{table}
        \centering
        
        \setlength{\tabcolsep}{3pt} %% default is 6pt
        \begin{tabular}{lrrrrrrrrrrrrr}
\toprule
	 & \textbf{QALD 1}  & \textbf{QALD 2}  & \textbf{QALD 3}  & \textbf{QALD 4}  & \textbf{QALD 5}  & \textbf{QALD 6}  & \textbf{QALD 7}  & \textbf{QALD 8}  & \textbf{QALD 9} & \textbf{QALD}  & \textbf{LC-QUAD}  & \textbf{Web} & \textbf{Graph}  \\ \midrule
	Cluster 1 & 18 & 14 & 14 & 16 & 18 & 20 & 21 & 21 & 20 & 17 & 37 & 40 & 20 \\ 
	Cluster 2 & 27 & 29 & 31 & 30 & 32 & 30 & 31 & 34 & 32 & 30 & 24 & 15 & 29 \\
	Cluster 3 & 52 & 52 & 51 & 44 & 45 & 44 & 36 & 36 & 42 & 45 & 20 & 40 & 30 \\ 
	Cluster 4 & 3 & 5 & 4 & 10 & 5 & 6 & 12 & 9 & 6 & 8 & 19 & 5 & 21 \\ \bottomrule
\end{tabular}
\captionof{table}{Question distribution (\%) clustered based on Detailed tags for each benchmark}% Add 'table' caption
        \label{table:detailed}
        \end{table}
        
        \begin{table}
        \centering
        
        \setlength{\tabcolsep}{3pt} %% default is 6pt
        \begin{tabular}{lrrrrrrrrrrrrr}
\toprule
	 & \textbf{QALD 1}  & \textbf{QALD 2}  & \textbf{QALD 3}  & \textbf{QALD 4}  & \textbf{QALD 5}  & \textbf{QALD 6}  & \textbf{QALD 7}  & \textbf{QALD 8}  & \textbf{QALD 9} & \textbf{QALD}  & \textbf{LC-QUAD}  & \textbf{Web} & \textbf{Graph}  \\ \midrule
	Cluster 1 & 26 & 21 & 22 & 18 & 21 & 22 & 18 & 22 & 21 & 20 & 16 & 25 & 13 \\ 
	Cluster 2 & 12 & 11 & 12 & 13 & 16 & 17 & 16 & 16 & 16 & 14 & 31 & 22 & 6 \\
	Cluster 3 & 14 & 21 & 20 & 17 & 18 & 18 & 17 & 20 & 19 & 18 & 13 & 11 & 25 \\ 
	Cluster 4 & 19 & 17 & 18 & 14 & 18 & 18 & 17 & 19 & 18 & 17 & 17 & 24 & 9 \\ 
	Cluster 5 & 21 & 17 & 16 & 18 & 17 & 16 & 14 & 14 & 16 & 15 & 13 & 16 & 14 \\ 
	Cluster 6 & 8 & 13 & 12 & 20 & 10 & 9 & 18 & 9 & 10 & 16 & 10 & 2 & 33 \\ \bottomrule
\end{tabular}
\captionof{table}{Question distribution (\%) clustered based on Dependency Parse Tree for each benchmark}% Add 'table' caption
          \label{table:parse}
        \end{table}  
        
    \end{scriptsize}
    \end{landscape}
%\clearpage% Flush page

==> sections/Results_questions_shapes.tex <==

\begin{table*}[t]
%\scriptsize
          
   \begin{tabular}{p{1cm}p{2cm}lp{6cm}}
\toprule
\multicolumn{1}{c}{\textbf{Shape}} & 
\multicolumn{1}{c}{\textbf{Question}} & 
\multicolumn{1}{c}{\textbf{Query}} & 
\multicolumn{1}{c}{\textbf{Graph}} \\
\midrule 
\emph{Single-Edge}	     
& 	Who discovered Pluto?		 
& 	
\begin{scriptsize}
\begin{lstlisting}[language=SPARQL, label=listing:query]
SELECT ?uri WHERE { 
    res:Pluto dbo:discoverer ?uri 
}
\end{lstlisting}
\end{scriptsize}
& \input{sections/ShapesExamples/Single}

\\
\midrule 
\emph{Chain}    
& 	Give me the capitals of all countries that the Himalayas run through.	 
& 	
\begin{scriptsize}
\begin{lstlisting}[language=SPARQL, label=listing:query]
SELECT DISTINCT ?uri WHERE { 
    res:Himalayas dbo:country ?country . 
    ?country dbo:capital ?uri 
}
\end{lstlisting}
\end{scriptsize}
& \input{sections/ShapesExamples/Chain} 
\\
\midrule 
\emph{Chain-Set, Forest}    
& 	Which building after the Burj Khalifa has the most floors?	 
& 	
\begin{scriptsize}
\begin{lstlisting}[language=SPARQL, label=listing:query]
SELECT DISTINCT ?uri WHERE { 
    res:Burj_Khalifa dbo:floorCount ?burj . 
    ?uri rdf:type dbo:Building . 
    ?uri dbo:floorCount ?proj 
    FILTER ( ?proj < ?burj ) 
} ORDER BY DESC(?proj) LIMIT 1
\end{lstlisting}
\end{scriptsize}
& \input{sections/ShapesExamples/Chain-Set}

\\
\midrule 
\emph{Tree, Star}    
& 	Who is the heaviest player of the Chicago Bulls?	 
& 	
\begin{scriptsize}
\begin{lstlisting}[language=SPARQL, label=listing:query]
SELECT DISTINCT ?uri WHERE { 
    ?uri a dbo:Person . 
    ?uri dbo:weight ?num 
    { ?uri dbp:team res:Chicago_Bulls } 
    UNION
    { ?uri dbp:draftTeam res:Chicago_Bulls } 
    UNION 
    { ?uri dbo:draftTeam res:Chicago_Bulls } 
} ORDER BY DESC(?num) OFFSET 0 LIMIT 1
\end{lstlisting}
\end{scriptsize}
& \input{sections/ShapesExamples/Tree}

\\
\midrule 
\emph{Cycle}    
& 	Which films starring Clint Eastwood did he direct himself?	 
& 	
\begin{scriptsize}
\begin{lstlisting}[language=SPARQL, label=listing:query]
SELECT DISTINCT ?uri WHERE {  
    ?uri dbo:director res:Clint_Eastwood .  
    ?uri dbo:starring res:Clint_Eastwood . 
}
\end{lstlisting}
\end{scriptsize}
& \input{sections/ShapesExamples/Cycle}


\\
\midrule 
\emph{Flower}    
& 	Which countries have more than ten caves?
& 	
\begin{scriptsize}
\begin{lstlisting}[language=SPARQL, label=listing:query]
SELECT DISTINCT ?uri WHERE { 
    ?uri a dbo:Country . 
    ?cave a dbo:Cave 
    { ?cave dbo:location ?uri } 
    UNION 
    { ?cave dbo:location ?loc . 
      ?loc dbo:country ?uri 
    } 
} GROUP BY ?uri HAVING ( COUNT(?cave) > 10 )
\end{lstlisting}
\end{scriptsize}
& \input{sections/ShapesExamples/Flower} \\

\midrule
\bottomrule%0
\\
\end{tabular}
\captionof{table}{A set of examples for the shapes used in \system. All the eamples are taken from QALD.}
\label{table:shapesExamples}
\end{table*}


==> sections/ShapesExamples/Chain-Set.tex <==

\begin{tiny}
\begin {tikzpicture}
[-latex ,auto ,node distance =1cm and 2cm ,
on grid , /tikz/overlay,
semithick ]

\node (A)  {$res:Burj\_Khalifa$};
\node (B) [right =of A] {$?burj$};

\node (C) [below =of B] {$?uri$};
\node (D) [right =of C] {$dbo:Building$};
\node (E) [left =of C] {$?proj$};

\path (A) edge [-, bend left =20] node[above =0.0 cm] 
{$dbo:floorCount$} (B);
\path (C) edge [-, bend left =20] node[above =0.0 cm] 
{$rdf:type$} (D);
\path (C) edge [-, bend right =20] node[above =-0.1 cm] 
{$dbo:floorCount$} (E);

\end{tikzpicture}
\end{tiny}


==> sections/ShapesExamples/Chain.tex <==

\begin{tiny}
\begin {tikzpicture}
[-latex ,auto ,node distance =1cm and 2cm ,
on grid , /tikz/overlay,
semithick ]

\node (A)  {$?uri$};
\node (B) [right =of A] {$?country$};
\node (C) [right =of B] {$Himalayas$};

\path (A) edge [-, bend left =20] node[above =0.0 cm] 
{$dbo:capital$} (B);
\path (B) edge [-, bend left =20] node[above =0.0 cm] 
{$dbo:country$} (C);

\end{tikzpicture}
\end{tiny}


==> sections/ShapesExamples/Cycle.tex <==

\begin{tiny}
\begin {tikzpicture}
[-latex ,auto ,node distance =1cm and 2cm ,
on grid , /tikz/overlay,
semithick ]

\node (A)  {$?uri$};
\node (B) [right =of A] {$res:Clint\_Eastwood$};

\path (A) edge [-, bend left =20] node[above =0.0 cm] 
{$dbo:director$} (B);
\path (A) edge [-, bend right =20] node[above =-0.3 cm] 
{$dbo:starring$} (B);

\end{tikzpicture}
\end{tiny}


==> sections/ShapesExamples/Flower.tex <==

\begin{tiny}
\begin {tikzpicture}
[-latex ,auto ,node distance =1cm and 2cm ,
on grid , /tikz/overlay,
semithick ]

\node (A)  {$dbo:Country$};
\node (B) [above right =of A] {$?uri$};
\node (C) [right =of A] {$?loc$};
\node (D) [right =of C] {$?cave$};
\node (E) [below =of D] {$dbo:Cave$};

\path (A) edge [-, bend left =20] node[above =0.0 cm] 
{$a$} (B);
\path (B) edge [-, bend left =20] node[above =-0.3 cm] 
{$dbo:country$} (C);
\path (B) edge [-, bend left =20] node[above =-0.1 cm] 
{$dbo:location$} (D);
\path (C) edge [-, bend right =20] node[above =-0.3 cm] 
{$dbo:location$} (D);
\path (D) edge [-, bend left =20] node[above =-0.1 cm] 
{$\ \ a$} (E);

\end{tikzpicture}
\end{tiny}


==> sections/ShapesExamples/Single.tex <==

\begin{tiny}
\begin {tikzpicture}
[-latex ,auto ,node distance =1 cm and 2cm ,
on grid , /tikz/overlay,
semithick ]

\node (B)  {$?uri$};
\node (C) [right =of B] {$res:Pluto$};

\path (B) edge [-, bend left =20] node[above =0.0 cm] 
{$dbo:discoverer$} (C);

\end{tikzpicture}
\end{tiny}


==> sections/ShapesExamples/Tree.tex <==

\begin{tiny}
\begin {tikzpicture}
[-latex ,auto ,node distance =1cm and 2cm ,
on grid , /tikz/overlay,
semithick ]

\node (A)  {$dbo:Person$};
\node (B) [above right =of A] {$?uri$};
\node (C) [right =of A] {$?num$};
\node (D) [below right =of C] {$res:Chicago_Bulls$};

\path (A) edge [-, bend left =20] node[above =0.0 cm] 
{$a$} (B);
\path (B) edge [-, bend left =20] node[above =-0.3 cm] 
{$dbo:weight$} (C);
\path (B) edge [-, bend left =20] node[above =0.0 cm, label={[align=left]a:dbp:team, \\
dbp:draftTeam,\\  
dbo:draftTeam}] 
{
} (D);

\end{tikzpicture}
\end{tiny}


==> sections/Systems.tex <==
\section{Systems}

There are many Question Answering system, however, most of them are not accessible at all. A portion of these systems are accessible through a web service. The systems that are collected for this analysis are:
\newcommand{\squishlist}{
  \begin{list}{$\bullet$}
   {
     \setlength{\itemsep}{0pt}
     \setlength{\parsep}{0pt}
     \setlength{\topsep}{0pt}
     \setlength{\partopsep}{0pt}
     \setlength{\leftmargin}{1.5em}
     \setlength{\labelwidth}{1em}
     \setlength{\labelsep}{0.5em} } }
\newcommand{\squishend}{
   \end{list}  }

\begin{squishlist}
    
    \item \textbf{gAnswer} ~\cite{hu2017answering}: GAnswer is a semantic query graph to model the query intention in the natural language question structurally, based on which, RDF QA is reduced to subgraph matching problem. The system is available online\footnote{\url{http://ganswer.gstore-pku.com}} and we evaluated it on the QALD-6 benchmark.
    
    \item \textbf{WDAqua-core1} ~\cite{diefenbach2018wdaqua}: This proposal does not concentrate on the syntax but on the semantics to analyze a question. This has essentially a couple of benefits: it works for both keyword and full natural language questions and it is multilingual. The system also is available online\footnote{\url{https://qanswer-frontend.univ-st-etienne.fr}} and we evaluated it on the QALD-9 benchmark.
    
    
    \item \textbf{TEQUILA} ~\cite{jia2018tequila}: TEQUILA is an enabler method for temporal QA that can run on top of any KBQA system. TEQUILA evaluated on the TempQuestions benchmark. 
    
    \item \textbf{QUEST} ~\cite{lu2019answering}: QUEST can answer complex questions directly from textual sources on-the-fly, by computing similarity joins over partial results from different documents. 
    
    \item \textbf{CONVEX} ~\cite{christmann2019look}: Convex is an unsupervised method that can answer incomplete questions over a knowledge graph (KG) by maintaining conversation context using entities and predicates seen so far and automatically inferring missing or ambiguous pieces for follow-up questions. Convex is evaluated on ConvQuestions.
    
    \item \textbf{QUINT} ~\cite{abujabal2017quint}: QUINT automatically learns role-aligned utterance-query templates from user questions paired with their answers. QUINT currently is not maintained and requires some efforts to make it works.
    
    \item \textbf{CANaLI} ~\cite{mazzeo2016canali}:    Context-Aware controlled Natural Language Interface (CANaL). CANaLI has been applied to QALD 6, however, it currently is not maintained and requires some efforts to make it works.
    
    

\end{squishlist}



==> sections/count_of_s-p-o.tex <==
%QALD all
551: [http://dbpedia.org/resource/The_Three_Dancers,
109: [http://dbpedia.org/property/locationCountry, 
255: [http://dbpedia.org/ontology/vicePresident,
Total::::: 915

%LC_QuAD
3815: [http://dbpedia.org/resource/Metallica
312: [http://dbpedia.org/property/type,
465: [http://dbpedia.org/ontology/formerPartner,
Total::::: 4592

